Semantic Communication for Task Execution and Data Reconstruction in Multi-View Scenarios

Semantic communication has gained significant attention with the advances in machine learning. Most semantic communication works focus on either task execution or data reconstruction, with some recent works combining the two. In this work, we propose a semantic communication system for concurrent task execution and data reconstruction for a multi-view scenario, which we formulate as the maximization of mutual information. To investigate the trade-off between the two objectives, we formulate a joint objective as a convex combination of task execution and data reconstruction. We show that under specific assumptions, the \ac{SSIM} loss can be obtained from the mutual information maximization objective for data reconstruction, which takes human visual perception into account. Furthermore, for constant resource use, we show that by increasing the weight of the reconstruction objective up to a certain point, the task execution performance can be kept nearly constant, while the data reconstruction can be significantly improved.

==> tikz/block_diagram/systemModel/4SplitImage.tex <==
\usetikzlibrary{shapes, arrows.meta, positioning}

\begin{tikzpicture}[auto, node distance=1.5cm and 1.5cm, thick, >=Stealth,
    block/.style={draw, rectangle, rounded corners, minimum width=3.5cm, minimum height=1.5cm, fill=orange!20},
    dashedblock/.style={draw, dashed, rectangle, rounded corners, minimum width=11cm, minimum height=7cm, fill=green!10},
    subblock/.style={draw,dashed, rectangle,rounded corners, minimum width=4.5cm, minimum height=1.5cm, fill=green!30},
    outputblock/.style={draw, rectangle, rounded corners, minimum width=3.5cm, minimum height=1.5cm, fill=blue!10},
    classblock/.style={draw, rectangle, rounded corners, minimum width=3.5cm, minimum height=1.5cm, fill=blue!20}
]

% Input image
\node[block, fill=orange!20, align=center,minimum width=6cm,minimum height=2cm] (semSource) {
  \huge \textbf{Semantic Source} \\[0.15cm]
  \fontsize{24pt}{32pt}\selectfont \textbf{$p(\mathbf{\bm s}, \mathbf{\bm z})$}
};

\node[right=2.5cm of semSource](input_img) {\includegraphics[width=2.5cm]{tikz/block_diagram/systemModel/splitImages/input_img-img0.png}};

% Input image
\node[block,fill=orange!20,align=center,right=2.5cm of input_img,minimum width=6cm,minimum height=2cm](split){\huge{\textbf{Image Splitter}}};

% Encoder
\node[block,dashed, fill=green!20,minimum width=6cm, right=3cm of split,align=center,minimum height=2cm] (encoder1) {\huge{\textbf{Encoder 1}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p_{\theta_n}(\bm x_1 \mid \bm s_1)}$}};

\node[block,dashed, fill=green!20,minimum width=6cm, below=1cm of encoder1,align=center,minimum height=2cm] (encoder2) {\huge{\textbf{Encoder 2}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p_{\theta_n}(\bm x_2 \mid \bm s_2)}$}};

\node[block,dashed, fill=green!20,minimum width=6cm, below=1cm of encoder2,align=center,minimum height=2cm] (encoder3) {\huge{\textbf{Encoder 3}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p_{\theta_n}(\bm x_3 \mid \bm s_3)}$}};

\node[block,dashed, fill=green!20,minimum width=6cm, below=1cm of encoder3,align=center,minimum height=2cm] (encoder4) {\huge{\textbf{Encoder $\mathbf{N_{\text{splits}}}$}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{\bm p_{\theta_n}(x_{N_{\text{splits}}} \mid \bm s_{N_{\text{splits}}})}$}};


% AWGN
\node[block, right=3cm of encoder1,minimum width=6cm,align=center,minimum height=2cm] (awgn1) {\huge{\textbf{Channel 1}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p(\bm y_1 \mid \bm x_1)}$}};

\node[block, below=1cm of awgn1,minimum width=6cm,align=center,minimum height=2cm] (awgn2) {\huge{\textbf{Channel 2}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p(\bm y_2 \mid \bm x_2)}$}};

\node[block, below=1cm of awgn2,minimum width=6cm,align=center,minimum height=2cm] (awgn3) {\huge{\textbf{Channel 3}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p(\bm y_3 \mid \bm x_3)}$}};

\node[block, below=1cm of awgn3,minimum width=6cm,align=center,minimum height=2cm] (awgn4) {\huge{\textbf{Channel $\mathbf{N_{\text{splits}}}$}} \\[0.15cm] \fontsize{20pt}{24pt}\selectfont \textbf{$\mathbf{p(\bm y_{N_{\text{splits}}} \mid \bm x_{N_{\text{splits}}})}$}};

% Decoder container
\node[dashedblock, below=2cm of encoder4, anchor=north] (decoder_box) {};

% Decoder label
\node[above=0.1cm of decoder_box.north] {\huge{\textbf{Decoder}}};

% Reconstruction decoder inside decoder box (top half)
\node[subblock, anchor=north, below=0.5cm of decoder_box.north,align=center,minimum width=6cm,minimum height=2cm] (rec_decoder) {\huge{\textbf{Reconstruction Dec}} \\[0.15cm] \fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{q_{\phi}(\bm s \mid \bm y)}$}};

% Classification decoder inside decoder box (bottom half)
\node[subblock, anchor=north, below=1cm of rec_decoder,align=center,minimum width=6cm,minimum height=2cm] (cls_decoder) {\huge{\textbf{Classification Dec}} \\[0.15cm] \fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{q_{\psi}(z \mid y)}$}};

\node[block, left=3cm of rec_decoder,align=center,minimum width=6cm,minimum height=2cm] (reconstruct) {\huge{\textbf{Rec. Decision}} \\[0.15cm] 
\fontsize{24pt}{28pt}\selectfont $\bm{\hat{s}} = \arg\max(\bm{q(s)})$};


\node[left=2cm of reconstruct] (output_img) {\includegraphics[width=2.5cm]{tikz/block_diagram/systemModel/splitImages/input_img-img0.png}};

% Classification path
\node[block, below= 0.95cm of reconstruct,align=center,minimum width=6cm,minimum height=2cm] (classification) {\huge{\textbf{Classific. Decision}} \\[0.15cm] 
\fontsize{24pt}{28pt}\selectfont $\bm{\hat{z}} = \arg\max(\bm{q(z)})$};

\node[left=of classification] (label) {\fontsize{24pt}{28pt}\selectfont \textbf{Frog}};

% Arrows from input to encoder to channel
\draw[->] (semSource)--(input_img);
\draw[->] (input_img) -- (split) node[midway, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{s}};

\foreach \n in {1,2,3,4} {
    \pgfmathtruncatemacro{\img}{\n}

    % Define label string
    \def\labeltext{}
    \ifnum\n=4
        \def\labeltext{\fontsize{24pt}{28pt}$\bm{s_{N_{\text{splits}}}}$}
    \else
        \def\labeltext{\fontsize{24pt}{28pt}$\bm{s_\n}$}
    \fi

    % Draw arrow
    \draw[->] 
        (split.east) -- ++(0.3,0)
        |- (encoder\n.west)
        node[pos=0.75, above, sloped] {
            \begin{tabular}{@{}c@{}}
                \labeltext \\
                \includegraphics[width=1.5cm]{tikz/block_diagram/systemModel/splitImages/split_image_\img-img0.png}
            \end{tabular}
        };
}

\draw[->] (encoder1.east) -- (awgn1.west) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm x_1}$}};
\draw[->] (encoder2.east) -- (awgn2.west) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm x_2}$}};
\draw[->] (encoder3.east) -- (awgn3.west) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm x_3}$}};
\draw[dotted,->] (encoder4.east) -- (awgn4.west) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm x_{N_{\text{splits}}}}$}};



% Decoder junction point
\coordinate (decoder_input) at ($(decoder_box.north east)+(0,-2.3)$);

\draw[->] 
  (awgn1.east) -- ($([xshift=2.75cm]awgn1.east)$) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm y_1}$}}
  -- ($([xshift=9.5cm]decoder_input.east)$)
  -- (decoder_input.east);

\draw[->] 
  (awgn2.east) -- ($([xshift=2.75cm]awgn2.east)$) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm y_2}$}}
  -- ($([xshift=9.5cm]decoder_input.east)$)
  -- (decoder_input.east);
  
\draw[->] 
  (awgn3.east) -- ($([xshift=2.75cm]awgn3.east)$) node[pos=0.5, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\bm y_3}$}}
  -- ($([xshift=9.5cm]decoder_input.east)$)
  -- (decoder_input.east);
  
\draw[dotted,->] 
  (awgn4.east) -- ($([xshift=2.75cm]awgn4.east)$) 
    node[pos=0.65, above, sloped] {\fontsize{24pt}{28pt}\selectfont $\mathbf{y_{N_{\text{splits}}}}$}
  -- ($([xshift=9.5cm]decoder_input.east)$)
  -- (decoder_input.east) 
    node[pos=0.45, below, sloped, align=center] {\fontsize{24pt}{28pt}\selectfont $\mathbf{y=[
  y_1^{\top} y_2^{\top} \dots y_{N_{\text{splits}}}^{\top}]^{\top}}$};


% Split to both decoders
\draw[->] (decoder_input) |- (rec_decoder.east) node[pos=0.75, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{y}$}};
\draw[->] (decoder_input) |- (cls_decoder.east) node[pos=0.75, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{y}$}};

\draw[->] (rec_decoder.west) -- (reconstruct) node[midway, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{q(s)}$}};

\draw[->] (reconstruct) -- (output_img) node[midway, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\hat{s}}$}};

\draw[->] (cls_decoder.west) -- (classification) node[midway, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{q(z)}$}};

\draw[->] (classification) -- (label) node[midway, above, sloped] {\fontsize{24pt}{28pt}\selectfont \textbf{$\mathbf{\hat{z}}$}};

\end{tikzpicture}


